An Efficient MPC Algorithm For Switched Systems with Minimum Dwell Time Constraints

This paper presents an efficient suboptimal model predictive control (MPC) algorithm for nonlinear switched systems subject to minimum dwell time constraints (MTC). While MTC are required for most physical systems due to stability, power and mechanical restrictions, MPC optimization problems with MTC are challenging to solve. To efficiently solve such problems, the on-line MPC optimization problem is decomposed into a sequence of simpler problems, which include two nonlinear programs (NLP) and a rounding step, as typically done in mixed-integer optimal control (MIOC). Unlike the classical approach that embeds MTC in a mixed-integer linear program (MILP) with combinatorial constraints in the rounding step, our proposal is to embed the MTC in one of the NLPs using move blocking. Such a formulation can speedup on-line computations by employing recent move blocking algorithms for NLP problems and by using a simple sum-up-rounding (SUR) method for the rounding step. An explicit upper bound of the integer approximation error for the rounding step is given. In addition, a combined shrinking and receding horizon strategy is developed to satisfy closed-loop MTC. Recursive feasibility is proven using a $l$-step control invariant ($l$-CI) set, where $l$ is the minimum dwell time step length. An algorithm to compute $l$-CI sets for switched linear systems off-line is also presented. Numerical studies show significant speed-up and comparable control performance of the proposed MPC algorithm against the classical approach, though at the cost of sub-optimal solutions.

==> Figure/Grid.tex <==
\begin{figure}[htb]
\centering
\begin{adjustbox}{max width=1\linewidth}{
\begin{tikzpicture}
\draw [<->](0,6)--(0,0)--(10,0);
\node [below] at (0,0) {$t_0$};
\draw [dashed,ultra thin] (1,0)--(1,6);
\draw [dashed,ultra thin] (2,0)--(2,6);
\draw [dashed,ultra thin] (3,0)--(3,6);
\node [below] at (1,0) {$t_{1}$};
\node [below] at (2,0) {$t_{2}$};
\node [below] at (3,0) {$t_{3}$};

\draw [dashed,ultra thin] (4,0)--(4,6);
\draw [dashed,ultra thin] (5,0)--(5,6);
\draw [dashed,ultra thin] (6,0)--(6,6);
\node [below] at (4,0) {$t_{4}$};
\node [below] at (5,0) {$t_{5}$};
\node [below] at (6,0) {$t_{6}$};

\draw [dashed,ultra thin] (7,0)--(7,6);
\draw [dashed,ultra thin] (8,0)--(8,6);
\draw [ultra thin] (9,0)--(9,6);
\node [below] at (7,0) {$t_{7}$};
\node [below] at (8,0) {$t_{8}$};
\node [below] at (9,0) {$t_{9}$};

\draw [fill=blue] (0,0.2) circle [radius=0.04];
\draw [thick, blue] (0,0.2) to [out=15,in=195] (1,1.2);
\draw [fill=blue] (1,0.2) circle [radius=0.04];
\draw [thick, blue] (1,0.2) to [out=15,in=195] (2,1.2);
\draw [fill=blue] (2,0.2) circle [radius=0.04];
\draw [thick, blue] (2,0.2) to [out=15,in=195] (3,1.2);
\draw [fill=blue] (2,0.2) circle [radius=0.04];
\draw [fill=blue] (3,0.2) circle [radius=0.04];
\draw [thick, blue] (3,0.2) to [out=15,in=195] (4,1.2);
\draw [fill=blue] (4,0.2) circle [radius=0.04];
\draw [thick, blue] (4,0.2) to [out=15,in=195] (5,1.2);
\draw [fill=blue] (5,0.2) circle [radius=0.04];
\draw [thick, blue] (5,0.2) to [out=15,in=195] (6,1.2);
\draw [fill=blue] (6,0.2) circle [radius=0.04];
\draw [thick, blue] (6,0.2) to [out=15,in=195] (7,1.2);
\draw [fill=blue] (7,0.2) circle [radius=0.04];
\draw [thick, blue] (7,0.2) to [out=15,in=195] (8,1.2);
\draw [fill=blue] (8,0.2) circle [radius=0.04];
\draw [thick, blue] (8,0.2) to [out=15,in=195] (9,1.2);
\draw [fill=blue] (9,0.2) circle [radius=0.04];

\node [xshift= -0.5cm] at (0,0.7) {$x(t)$};

\draw [dashed, ultra thin] (0,2)--(1,2);
\draw [dashed, ultra thin] (1,2.5)--(2,2.5);
\draw [dashed, ultra thin] (2,1.8)--(3,1.8);
\draw [dashed, ultra thin] (3,2.2)--(4,2.2);
\draw [dashed, ultra thin] (4,2.6)--(5,2.6);
\draw [dashed, ultra thin] (5,2.8)--(6,2.8);
\draw [dashed, ultra thin] (6,1.9)--(7,1.9);
\draw [dashed, ultra thin] (7,2.3)--(8,2.3);
\draw [dashed, ultra thin] (8,2.0)--(9,2.0);

\node [xshift= -0.5cm] at (0,2) {$u(t)$};

\draw [red] (0,4)--(1,4);
\draw [red] (1,5)--(2,5);
\draw [red] (2,5)--(3,5);
\draw [ultra thin, red] (3,4)--(4,4);
\draw [ultra thin, red] (4,5)--(5,5);
\draw [ultra thin, red] (5,4)--(6,4);
\draw [ultra thin, red] (6,4)--(7,4);
\draw [ultra thin, red] (7,4)--(8,4);
\draw [ultra thin, red] (8,5)--(9,5);

\draw [ultra thin, red] (1,4)--(1,5);
\draw [ultra thin, red] (3,4)--(3,5);
\draw [ultra thin, red] (4,4)--(4,5);
\draw [ultra thin, red] (5,4)--(5,5);
\draw [ultra thin, red] (8,4)--(8,5);


\node [xshift= -0.5cm] at (0,4) {$b_1(t)$};

\node [xshift= 0.5cm] at (9,4) {$0$};
\node [xshift= 0.5cm] at (9,5) {$1$};

\end{tikzpicture}
}
\end{adjustbox}
\caption{An illustration of the discretization of the state, control and switching sequence trajectories when $\mathbb{Q}=\{1,2\}$ and $N=9$.}
\label{fig:mygrid}
\end{figure}

==> Figure/Grid_M.tex <==
\begin{figure}[htb]
\centering
\begin{adjustbox}{max width=1\linewidth}{
\begin{tikzpicture}
\draw [<->](0,5)--(0,0)--(9.5,0);
\draw (-0.5,0)--(0,0);
\node [below] at (0,0) {$\tau_{0,1}$};
\draw [ultra thin] (1,-0.2)--(1,0.2);
\draw [ultra thin] (2,-0.2)--(2,0.2);
\draw [ultra thin] (3,-0.2)--(3,0.2);
\node [xshift=-0.2cm,below] at (1,-0.2) {$\tau_{0,1}^1$};
\node [xshift=-0.2cm,below] at (2,-0.2) {$\tau_{0,1}^2$};
\node [xshift=-0.2cm,below] at (3,-0.2) {$\tau_{0,1}^3$};


\draw [ultra thin] (4,-0.2)--(4,0.2);
\draw [ultra thin] (5,-0.2)--(5,0.2);
\draw [ultra thin] (6,-0.2)--(6,0.2);
\node [xshift=-0.1cm,below] at (4,-0.2) {$\tau_{0,1}^4$};
\node [xshift=-0.1cm,below] at (5,-0.2) {$\tau_{0,1}^5$};
\node [xshift=-0.1cm,below] at (6,-0.2) {$\tau_{0,1}^6$};

\draw [ultra thin] (7,-0.2)--(7,0.2);
\draw [ultra thin] (8,-0.2)--(8,0.2);
\node [xshift=0.2cm,below] at (7,-0.2) {$\tau_{0,1}^7$};
\node [xshift=0.2cm,below] at (8,-0.2) {$\tau_{0,1}^8$};

\draw [ultra thin] (9,0)--(9,5);
\node [xshift= 0.1cm,below] at (9,0) {$\tau_{0,2}$};

\draw [fill=blue] (0,0.2) circle [radius=0.04];
\draw [thick, blue] (0,0.2) to [out=15,in=195] (1,1.2);
\draw [fill=blue] (1,0.2) circle [radius=0.04];
\draw [thick, blue] (1,0.2) to [out=15,in=195] (2,1.2);
\draw [fill=blue] (2,0.2) circle [radius=0.04];
\draw [thick, blue] (2,0.2) to [out=15,in=195] (3,1.2);
\draw [fill=blue] (2,0.2) circle [radius=0.04];
\draw [fill=blue] (3,0.2) circle [radius=0.04];
\draw [thick, blue] (3,0.2) to [out=15,in=195] (4,1.2);
\draw [fill=blue] (4,0.2) circle [radius=0.04];
\draw [thick, blue] (4,0.2) to [out=15,in=195] (5,1.2);
\draw [fill=blue] (5,0.2) circle [radius=0.04];
\draw [thick, blue] (5,0.2) to [out=15,in=195] (6,1.2);
\draw [fill=blue] (6,0.2) circle [radius=0.04];
\draw [thick, blue] (6,0.2) to [out=15,in=195] (7,1.2);
\draw [fill=blue] (7,0.2) circle [radius=0.04];
\draw [thick, blue] (7,0.2) to [out=15,in=195] (8,1.2);
\draw [fill=blue] (8,0.2) circle [radius=0.04];
\draw [thick, blue] (8,0.2) to [out=15,in=195] (9,1.2);
\draw [fill=blue] (9,0.2) circle [radius=0.04];

\node [xshift= -0.5cm] at (0,0.7) {$x(t)$};

\draw [dashed, ultra thin] (0,2)--(1,2);
\draw [dashed, ultra thin] (1,2.5)--(2,2.5);
\draw [dashed, ultra thin] (2,1.8)--(3,1.8);
\draw [dashed, ultra thin] (3,2.2)--(4,2.2);
\draw [dashed, ultra thin] (4,2.6)--(5,2.6);
\draw [dashed, ultra thin] (5,2.8)--(6,2.8);
\draw [dashed, ultra thin] (6,1.9)--(7,1.9);
\draw [dashed, ultra thin] (7,2.3)--(8,2.3);
\draw [dashed, ultra thin] (8,2.0)--(9,2.0);

\node [xshift= -0.5cm] at (0,2.5) {$u(t)$};

\draw [ultra thin] (0,4)--(9,4);
\node [above] at (4.3,4) {$2$};


\node [xshift= -0.5cm] at (0,4) {$q(t)$};

\end{tikzpicture}
}
\end{adjustbox}
\caption{An illustration of the separate discretization of the state, control and switching sequence trajectories in $(\tau_{0,1},\tau_{0,2})$ in Fig. \ref{fig:mygrid} for $M=9$.}
\label{fig:mygrid_M}
\end{figure}
